Rethinking Data Augmentation for Robust LiDAR Semantic Segmentation in Adverse Weather

Existing LiDAR semantic segmentation methods often struggle with performance declines in adverse weather conditions. Previous work has addressed this issue by simulating adverse weather or employing universal data augmentation during training. However, these methods lack a detailed analysis and understanding of how adverse weather negatively affects LiDAR semantic segmentation performance. Motivated by this issue, we identified key factors of adverse weather and conducted a toy experiment to pinpoint the main causes of performance degradation: (1) Geometric perturbation due to refraction caused by fog or droplets in the air and (2) Point drop due to energy absorption and occlusions. Based on these findings, we propose new strategic data augmentation techniques. First, we introduced a Selective Jittering (SJ) that jitters points in the random range of depth (or angle) to mimic geometric perturbation. Additionally, we developed a Learnable Point Drop (LPD) to learn vulnerable erase patterns with a Deep Q-Learning Network to approximate the point drop phenomenon from adverse weather conditions. Without precise weather simulation, these techniques strengthen the LiDAR semantic segmentation model by exposing it to vulnerable conditions identified by our data-centric analysis. Experimental results confirmed the suitability of the proposed data augmentation methods for enhancing robustness against adverse weather conditions. Our method achieves a notable 39.5 mIoU on the SemanticKITTI-to-SemanticSTF benchmark, improving the baseline by 8.1\%p and establishing a new state-of-the-art. Our code will be released at \url{https://github.com/engineerJPark/LiDARWeather}.

==> supp_table/ablation_hyperparam.tex <==
\begin{table}[h]
    \centering
    \caption{\footnotesize{Hyperparameter ablation in SemanticKITTI-to-SemanticSTF. The values we chose are highlighted in \textbf{bold}.}}
    \label{tab:ablation_all}
    \begin{subtable}{0.45\linewidth}
        \centering
        \begin{minipage}{\linewidth}
            \centering
            \scalebox{0.75}{
            \begin{tabular}{cccccc}
                \toprule
                \multicolumn{6}{c}{Selective Jittering}  \\
                DSJ range & mIoU & ASJ $\Delta\theta$ & mIoU & Gaussian $\sigma$ & mIoU \\
                \midrule
                $\left[2,5\right]$ & 39.3 & $\frac{1}{2}\pi$ & 38.1 & 0.001 & 37.5 \\
                $\left[3,6\right]$ & 38.8 & $\frac{3}{4}\pi$ & 39.9 & 0.005 & 38.4  \\
                $\left[4,7\right]$ & 37.8 & \textbf{$\pi$} & \textbf{39.5} & \textbf{0.01} & \textbf{39.5} \\
                \textbf{[5,8]} & \textbf{39.5} & $\frac{5}{4}\pi$ & 40.0 & 0.05 & 37.3 \\
                $\left[6,9\right]$ & 37.8 & $\frac{3}{2}\pi$ & 39.3 & 0.1 & 37.9  \\
                \midrule
                {\footnotesize deviation} &  0.8 & {\footnotesize deviation} & 0.2 & {\footnotesize deviation} & 1.3 \\
            \bottomrule
            \end{tabular}
            }
        \end{minipage}
    \end{subtable}
    \hspace{0.05\linewidth} % Adjust the space between subtables
    \begin{subtable}{0.45\linewidth}
        \centering
        \begin{minipage}{\linewidth}
            \centering\scalebox{0.75}{
            \begin{tabular}{cccccc}
                \toprule
                \multicolumn{6}{c}{Learable Point Drop} \\
                 Batch size & mIoU & Discount $\gamma$ & mIoU & Decay $\epsilon$ & mIoU\\
                \midrule
                8 & 37.1 & 0.5 & 37.8 & 100 & 38.5 \\
                16 & 37.1 & 0.8 & 38.4 & 500 & 38.7 \\
                \textbf{32} & \textbf{39.5} & 0.9 & 38.4 & \textbf{1000} & \textbf{39.5} \\
                64 & 38.2 & \textbf{0.99} & \textbf{39.5} & 2000 & 37.3 \\
                128 & 37.0 & 0.999 & 38.8 & 3000 & 40.3 \\
                \midrule
                {\footnotesize deviation} &  1.7 & {\footnotesize deviation} & 0.9 & {\footnotesize deviation} & 0.7 \\
            \bottomrule
            \end{tabular}}
        \end{minipage}
    \end{subtable}
\label{tab:ablation_hyperparam}
\end{table}


==> supp_table/asjdsj_analysis.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[h]
\centering
\caption{Experiments on ASJ/DSJ relative to all-point jittering/CSJ. All models were trained on SemanticKITTI and validated on SemanticSTF. The values in parentheses indicate the performance improvement or decrease over the baseline model.}
\begin{footnotesize}
\begin{tabular}{l|c|cccc|c}
        \toprule
        Methods & \rotatebox{90}{Clean} & \rotatebox{90}{D-fog} & \rotatebox{90}{L-fog} &  \rotatebox{90}{Rain} & \rotatebox{90}{Snow} & mIoU \\
    \midrule
    Baseline & \textbf{63.9} & 30.7 & 30.1 & 29.7 & 25.3 & 31.4 \\
    Jittering & 61.7 {\tiny \textcolor{blue}{(-2.2)}} & \underline{34.3} & \underline{36.3} & 33.2 & \textbf{32.4} & \underline{36.9} {\tiny \textcolor{red}{(+5.5)}} \\
    CSJ & \underline{63.2} {\tiny \textcolor{blue}{(-0.7)}} & 32.9 & 31.1 & 28.8 & 23.2 & 31.2 {\tiny \textcolor{blue}{(-0.2)}} \\
    \midrule
    ASJ & 62.1 {\tiny \textcolor{blue}{(-1.8)}} & 33.3 & 35.4 & \textbf{37.8} & \underline{31.6} & 36.8 {\tiny \textcolor{red}{(+5.4)}} \\
    DSJ & 62.2  {\tiny \textcolor{blue}{(-1.7)}}& \textbf{34.6} & \textbf{36.8} & \underline{36.1} & 31.2 & \textbf{38.0} {\tiny \textcolor{red}{(+6.6)}} \\
    \bottomrule
\end{tabular}
\label{tab:asjdsj_analysis}
\end{footnotesize}
\end{table}



==> supp_table/class_iou_semantickitti.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[ht]
\centering
\caption{LiDAR segmentation results (mIoU) on the SemanticSTF validation set of models trained with SemanticKITTI. D-fog and L-fog denote dense fog and light fog weather conditions in all experiments. $^\ast$ is the reproduced result with the same segmentation backbone. The best score is in \textbf{bold} and the second best is \underline{underlined}.}
\scalebox{0.65}{
\begin{tabular}{l|ccccccccccccccccccc|c}
    \toprule
    Methods & \rotatebox{90}{car} & \rotatebox{90}{bi.cle} & \rotatebox{90}{mt.cle} & \rotatebox{90}{truck} & \rotatebox{90}{oth-v.} & \rotatebox{90}{pers.} & \rotatebox{90}{bi.clst} & \rotatebox{90}{mt.clst} & \rotatebox{90}{road} & \rotatebox{90}{parki.} & \rotatebox{90}{sidew.} & \rotatebox{90}{oth-g.} & \rotatebox{90}{build.} & \rotatebox{90}{fence} & \rotatebox{90}{veget.} & \rotatebox{90}{trunk} & \rotatebox{90}{terra.} & \rotatebox{90}{pole} & \rotatebox{90}{traf.} & mIoU \\
    \midrule
    Oracle & 89.4 & 42.1 & 0.0 & 59.9 & 61.2 & 69.6 & 39.0 & 0.0 & 82.2 & 21.5 & 58.2 & 45.6 & 86.1 & 63.6 & 80.2 & 52.0 & 77.6 & 50.1 & 61.7 & 54.7\\ 
    \midrule
    Baseline & 67.1 & \underline{5.0} & \textbf{28.1} & 38.5 & \underline{14.6} & 45.8 & 8.3 & 13.8 & 40.1 & \textbf{16.1} & 26.1 & 3.3 & 71.6 & \textbf{52.7} & 53.8 & 33.9 & 39.2 & \underline{25.3} & 12.7 & 31.4 \\
    LaserMix \cite{kong_lasermix_2023} & 18.6 & \textbf{5.4} & 0.0 & 9.9 & 1.6 & 0.6 & 7.9 & 10.5 & 47.6 & 6 & 12.1 & 1.8 & 21.6 & 20.2 & 48.4 & 6.6 & 37.8 & 19 & 2.8 & 14.7 \\
    PolarMix \cite{xiao_polarmix_nodate} & 21 & 2 & 0.0 & 3.8 & 1.6 & 2.8 & 0.6 & 0.0 & \underline{58.3} & 4.4 & 17.4 & 1.4 & 40.7 & 36.4 & 41.3 & 6.6 & 35 & 14.6 & 2.8 & 15.3 \\
    PointDR$^\ast$ \cite{xiao_3d_2023} & \underline{69.2} & 1 & 8.9 & \textbf{41.9} & 7.6 & \underline{48.9} & \textbf{17.0} & \underline{36.2} & 57.8 & \underline{15.9} & \underline{32.3} & \underline{4.0} & \textbf{75.7} & 46.4 & \underline{54.0} & \underline{36.2} & \underline{43.9} & 23.7 & \underline{24.2} & \underline{33.9} \\
    \midrule
    Baseline+SJ+LPD & \textbf{86.1} & 4.8 & \underline{13.8} & \underline{39.7} & \textbf{26.6} & \textbf{55.4} & \underline{8.5} & \textbf{50.4} & \textbf{63.7} & 14.9 & \textbf{37.9} & \textbf{5.5} & \underline{75.2} & \textbf{52.7} & \textbf{60.4} & \textbf{39.7} & \textbf{44.9} & \textbf{30.1} & \textbf{40.8} & \textbf{39.5} \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+19.0}} & {\scriptsize \textcolor{blue}{-0.2}} & {\scriptsize \textcolor{blue}{-14.3}} & {\scriptsize \textcolor{red}{+1.1}} & {\scriptsize \textcolor{red}{+12.0}} & {\scriptsize \textcolor{red}{+9.6}} & {\scriptsize \textcolor{red}{+0.2}} & {\scriptsize \textcolor{red}{+36.6}} & {\scriptsize \textcolor{red}{+23.5}} & {\scriptsize \textcolor{blue}{-1.2}} & {\scriptsize \textcolor{red}{+11.9}} & {\scriptsize \textcolor{red}{+2.2}} & {\scriptsize \textcolor{red}{+3.6}} & 0.0 & {\scriptsize \textcolor{red}{+6.7}} & {\scriptsize \textcolor{red}{+5.8}} & {\scriptsize \textcolor{red}{+5.7}} & {\scriptsize \textcolor{red}{+4.9}} & {\scriptsize \textcolor{red}{+28.2}} & {\scriptsize \textcolor{red}{+8.1}} \\
    \bottomrule
\end{tabular}
}
\label{tab:supp_classiou_semantickitti}
\end{table}



==> supp_table/class_iou_synlidar.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[h]
\centering
\caption{LiDAR segmentation results (mIoU) on the SemanticSTF validation set of models trained with SynLiDAR. D-fog and L-fog denote dense fog and light fog weather conditions in all experiments. $^\ast$ is the reproduced result with the same segmentation backbone. The symbol $\ddagger$ indicates that the validation for model selection was performed on sequence 0 of SynLiDAR, rather than SemanticSTF. The best score is in \textbf{bold} and the second best is \underline{underlined}.}
\scalebox{0.58}{
\begin{tabular}{l|ccccccccccccccccccc|c}
    \toprule
    Methods & \rotatebox{90}{car} & \rotatebox{90}{bi.cle} & \rotatebox{90}{mt.cle} & \rotatebox{90}{truck} & \rotatebox{90}{oth-v.} & \rotatebox{90}{pers.} & \rotatebox{90}{bi.clst} & \rotatebox{90}{mt.clst} & \rotatebox{90}{road} & \rotatebox{90}{parki.} & \rotatebox{90}{sidew.} & \rotatebox{90}{oth-g.} & \rotatebox{90}{build.} & \rotatebox{90}{fence} & \rotatebox{90}{veget.} & \rotatebox{90}{trunk} & \rotatebox{90}{terra.} & \rotatebox{90}{pole} & \rotatebox{90}{traf.} & mIoU \\
    \midrule
    Oracle & 89.4 & 42.1 & 0.0 & 59.9 & 61.2 & 69.6 & 39.0 & 0.0 & 82.2 & 21.5 & 58.2 & 45.6 & 86.1 & 63.6 & 80.2 & 52.0 & 77.6 & 50.1 & 61.7 & 54.7\\ 
    \midrule
    Baseline & 33.76 & 1.71 & \underline{3.29} & 15.54 & 0.24 & 25.52 & 1.65 & 3.43 & 15.27 & 9.16 & 16.76 & 0.05 & 33.38 & 21.89 & 39.49 & 18.7 & \textbf{44.03} & 8.75 & 0.84 & 15.45 \\
    LaserMix \cite{kong_lasermix_2023} & \textbf{52.41} & \textbf{5.6} & 1.05 & 7.91 & \underline{1.96} & 25.59 & 1.62 & 2.92 & \textbf{44.58} & 6.44 & \underline{21.21} & 0.88 & 16.95 & 23.61 & 40.75 & 18.91 & 41.45 & 5.65 & 0.7 & 16.85 \\
    PolarMix \cite{xiao_polarmix_nodate} & \underline{48.93} & \underline{4.23} & 2.32 & 14.64 & \textbf{2.37} & 24.55 & 2.14 & 4.64 & 34.64 & 7.66 & 19.8 & 0.39 & 37.44 & 22.3 & 44.85 & 21.32 & \underline{43.18} & 7.08 & 1.3 & 18.09 \\
    PointDR$^\ast$ \cite{xiao_3d_2023} & 41.07 & 2.81 & \textbf{3.43} & 18.05 & 0.17 & \textbf{31.3} & \textbf{2.81} & 3.3 & 34.39 & \textbf{10.23} & 19.72 & \underline{0.96} & \textbf{52.72} & 21.98 & \textbf{48.49} & 21.33 & 38.31 & 19.19 & 5.61 & 19.78 \\
    PointDR$^\ast$$\ddagger$ \cite{xiao_3d_2023} & 36.13 & 3.47 & 2.15 & \textbf{21.93} & 0.31 & 28.72 & 1.69 & \textbf{5.09} & \underline{42.92} & 9.31 & 20.71 & 0.58 & 50.83 & \underline{26.88} & 46.85 & \textbf{24.49} & 37.69 & \underline{22.74} & 6.45 & \underline{20.47} \\
    \midrule
    Baseline+SJ+LPD & 42.13 & 2.79 & 2.68 & 19.22 & 0.67 & \underline{29.22} & 1.91 & \underline{4.8} & 42.32 & 8.67 & 21.05 & \textbf{1.56} & 48.23 & 25.97 & 47.17 & 22.11 & 32.8 & 21.74 & \underline{6.54} & 20.08 \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+8.4}} & {\scriptsize \textcolor{red}{+1.1}} & {\scriptsize \textcolor{blue}{-0.6}} & {\scriptsize \textcolor{red}{+3.7}} & {\scriptsize \textcolor{red}{+0.4}} & {\scriptsize \textcolor{red}{+3.7}} & {\scriptsize \textcolor{red}{+0.3}} & {\scriptsize \textcolor{red}{+1.4}} & {\scriptsize \textcolor{red}{+27.0}} & {\scriptsize \textcolor{blue}{-0.5}} & {\scriptsize \textcolor{red}{+4.3}} & {\scriptsize \textcolor{red}{+1.5}} & {\scriptsize \textcolor{red}{+14.9}} & {\scriptsize \textcolor{red}{+4.1}} & {\scriptsize \textcolor{red}{+7.7}} & {\scriptsize \textcolor{red}{+3.4}} & {\scriptsize \textcolor{blue}{-11.2}} & {\scriptsize \textcolor{red}{+13.0}} & {\scriptsize \textcolor{red}{+5.7}} & {\scriptsize \textcolor{red}{+4.6}} \\
    Baseline+SJ+LPD$\ddagger$ & 39.26 & 2.89 & 0.89 & \underline{19.39} & 0.75 & 27.68 & \underline{2.19} & 3.78 & 42.5 & \underline{9.35} & \textbf{21.55} & 0.3 & \underline{51.89} & \textbf{33.48} & \underline{47.38} & \underline{23.11} & 33.31 & \textbf{23.22} & \textbf{6.78} & \textbf{20.51} \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+5.5}} & {\scriptsize \textcolor{red}{+1.2}} & {\scriptsize \textcolor{blue}{-2.4}} & {\scriptsize \textcolor{red}{+3.8}} & {\scriptsize \textcolor{red}{+0.5}} & {\scriptsize \textcolor{red}{+2.2}} & {\scriptsize \textcolor{red}{+0.5}} & {\scriptsize \textcolor{red}{+0.4}} & {\scriptsize \textcolor{red}{+27.2}} & {\scriptsize \textcolor{red}{+0.2}} & {\scriptsize \textcolor{red}{+4.8}} & {\scriptsize \textcolor{red}{+0.3}} & {\scriptsize \textcolor{red}{+18.5}} & {\scriptsize \textcolor{red}{+11.6}} & {\scriptsize \textcolor{red}{+7.9}} & {\scriptsize \textcolor{red}{+4.4}} & {\scriptsize \textcolor{blue}{-10.7}} & {\scriptsize \textcolor{red}{+14.5}} & {\scriptsize \textcolor{red}{+5.9}} & {\scriptsize \textcolor{red}{+5.1}} \\
    \bottomrule
\end{tabular}
}
\label{tab:supp_classiou_synlidar}
\end{table}



==> supp_table/cosmix_unimix.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison with CosMix and UniMix. DA and DG denote domain adaptation and domain generalization.}
    \begin{tabular}{cc}
        \toprule
        Methods &  mIoU \\
        \midrule
        CoSMix(DA) & 28.4 \\
        UniMix(DA) & 37.2 \\
        UniMix(DG) & 31.4 \\
        \midrule
        MinkowskiNet18+Ours & 36.3 \\
        \bottomrule
    \end{tabular}
\label{tab:compare_dgda}
\end{table}

==> supp_table/mIoU_synlidar.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[ht]
\centering
\caption{LiDAR segmentation results (mIoU) on the SemanticSTF~\cite{xiao_3d_2023} \textit{validation set} of models trained with SemanticSTF~\cite{xiao_3d_2023}. $^\ast$ is the reproduced result with the same segmentation backbone. The symbol $\ddagger$ indicates that the validation for model selection was performed on sequence 0 of SynLiDAR, rather than SemanticSTF. The best score is in \textbf{bold} and the second best is \underline{underlined}.}
\scalebox{0.9}{
\begin{tabular}{l|cccc|c}
    \toprule
    Methods & \rotatebox{90}{D-fog} & \rotatebox{90}{L-fog} &  \rotatebox{90}{Rain} & \rotatebox{90}{Snow} & mIoU \\
    \midrule
    Oracle & 51.9 & 54.6 & 57.9 & 53.7 & 54.7\\ 
    \midrule
    Baseline & 15.24 & 15.97 & 16.83 & 12.76 & 15.45 \\
    LaserMix \cite{kong_lasermix_2023} & 15.32 & 17.95 & 18.55 & 13.8 & 16.85 \\
    PolarMix \cite{xiao_polarmix_nodate} & 16.47 & 18.69 & 19.63 & 15.98 & 18.09 \\
    PointDR$^\ast$ \cite{xiao_3d_2023}& \underline{19.09} & 20.28 & \underline{25.29} & \underline{18.98} & 19.78 \\
    PointDR$^\ast$$\ddagger$ & \textbf{21.41} & \underline{20.94} & \textbf{25.48} & \textbf{19.31} & \underline{20.47} \\
    \midrule
    Baseline+SJ+LPD & 19.08 & 20.65 & 21.97 & 17.27 & 20.08 \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+3.8}} & {\scriptsize \textcolor{red}{+4.7}} & {\scriptsize \textcolor{red}{+5.1}} & {\scriptsize \textcolor{red}{+4.5}} & {\scriptsize \textcolor{red}{+4.6}} \\
    Baseline+SJ+LPD$\ddagger$ & 18.99 & \textbf{21.22} & 23.14 & 17.28 & \textbf{20.51} \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+3.7}} & {\scriptsize \textcolor{red}{+5.3}} & {\scriptsize \textcolor{red}{+6.3}} & {\scriptsize \textcolor{red}{+4.5}} & {\scriptsize \textcolor{red}{+5.1}} \\
    \bottomrule
\end{tabular}
}
\label{tab:main_synlidar}
\end{table}

==> supp_table/toyex.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[h]
\centering
\caption{Results of toy experiments from \textit{validation set} of SynLIDAR~\cite{xiao_transfer_2022}.}
\begin{footnotesize}
\scalebox{0.7}{
\begin{tabular}{l|ccccccccccccccccccc|c}
    \toprule
    Methods & \rotatebox{90}{car} & \rotatebox{90}{bi.cle} & \rotatebox{90}{mt.cle} & \rotatebox{90}{truck} & \rotatebox{90}{oth-v.} & \rotatebox{90}{pers.} & \rotatebox{90}{bi.clst} & \rotatebox{90}{mt.clst} & \rotatebox{90}{road} & \rotatebox{90}{parki.} & \rotatebox{90}{sidew.} & \rotatebox{90}{oth-g.} & \rotatebox{90}{build.} & \rotatebox{90}{fence} & \rotatebox{90}{veget.} & \rotatebox{90}{trunk} & \rotatebox{90}{terra.} & \rotatebox{90}{pole} & \rotatebox{90}{traf.} & mIoU \\
    \midrule
    Clean & 0.0 & 54.9 & 94.1 & 0.0 & 0.0 & 94.8 & 93.7 & 0.0 & 94.8 & 0.0 & 89.8 & 0.0 & 98.2 & 53.7 & 76.8 & 90.3 & 0.0 & 86 & 95.2 & 53.8 \\
    \midrule
    \textbf{D1} : soft & 0.0 & 37.0 & 86.7 & 0.0 & 0.0 & 89.5 & 87.8 & 0.0 & 92.6 & 0.0 & 85.1 & 0.0 & 93.8 & 32.4 & 39.5 & 80.9 & 0.0 & 84.7 & 93.0 & 50.2 \\
    \textbf{D1} : hard & 0.0 & 9.1 & 53.9 & 0.0 & 0.0 & 56.0 & 48.6 & 0.0 & 20.9 & 0.0 & 23.7 & 0.0 & 31.0 & 0.4 & 4.8 & 26.7 & 0.0 & 39.6 & 74.4 & \textbf{21.6} \\
    \textbf{D2} : soft & 0.0 & 4.2 & 86.7 & 0.0 & 0.0 & 88.2 & 87.8 & 0.0 & 92.5 & 0.0 & 48.4 & 0.0 & 52.1 & 7.0 & 1.4 & 68.8 & 0.0 & 28.8 & 26.8 & 31.2 \\
    \textbf{D2} : hard & 0.0 & 0.2 & 52.5 & 0.0 & 0.0 & 50.3 & 48.4 & 0.0 & 20.6 & 0.0 & 3.1 & 0.0 & 4.0 & 0.2 & 0.1 & 10.5 & 0.0 & 2.2 & 8.7 & \textbf{11.1} \\
    \textbf{D3} : soft & 0.0 & 55.7 & 79.6 & 0.0 & 0.0 & 86.5 & 87.4 & 0.0 & 45.0 & 0.0 & 50.4 & 0.0 & 55.3 & 22.3 & 6.8 & 74.1 & 0.0 & 69.5 & 29.1 & 34.8 \\
    \textbf{D3} : hard & 0.0 & 12.5 & 11.3 & 0.0 & 0.0 & 63.3 & 32.9 & 0.0 & 0.2 & 0.0 & 3.5 & 0.0 & 6.6 & 1.9 & 2.8 & 45.6 & 0.0 & 4.1 & 0.1 & \textbf{9.7} \\
    \textbf{D4} : soft & 0.0 & 54.8 & 94.1 & 0.0 & 0.0 & 94.8 & 93.8 & 0.0 & 94.8 & 0.0 & 89.8 & 0.0 & 98.2 & 53.8 & 76.6 & 90.2 & 0.0 & 86 & 95.2 & 53.8 \\
    \textbf{D4} : hard & 0.0 & 54.8 & 94.1 & 0.0 & 0.0 & 94.8 & 93.8 & 0.0 & 94.8 & 0.0 & 89.8 & 0.0 & 98.2 & 53.8 & 76.6 & 90.2 & 0.0 & 86 & 95.2 & 53.8 \\
    \bottomrule
\end{tabular}
}
\label{tab:supplementary_toyex}
\end{footnotesize}
\end{table}


==> table/Ablation2.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[t]
\centering
\caption{Experiments on ASJ/DSJ relative to all-point jittering/CSJ. All models were trained on SemanticKITTI and validated on SemanticSTF. The values in parentheses indicate the performance improvement or decrease over the baseline model.}
\begin{footnotesize}
\begin{tabular}{l|c|cccc|c}
        \toprule
        Methods & \rotatebox{90}{Clean} & \rotatebox{90}{D-fog} & \rotatebox{90}{L-fog} &  \rotatebox{90}{Rain} & \rotatebox{90}{Snow} & mIoU \\
    \midrule
    Baseline & \textbf{63.9} & 30.7 & 30.1 & 29.7 & 25.3 & 31.4 \\
    Jittering & 61.7 {\tiny \textcolor{blue}{(-2.2)}} & \underline{34.3} & \underline{36.3} & 33.2 & \textbf{32.4} & \underline{36.9} {\tiny \textcolor{red}{(+5.5)}} \\
    CSJ & \underline{63.2} {\tiny \textcolor{blue}{(-0.7)}} & 32.9 & 31.1 & 28.8 & 23.2 & 31.2 {\tiny \textcolor{blue}{(-0.2)}} \\
    \midrule
    ASJ & 62.1 {\tiny \textcolor{blue}{(-1.8)}} & 33.3 & 35.4 & \textbf{37.8} & \underline{31.6} & 36.8 {\tiny \textcolor{red}{(+5.4)}} \\
    DSJ & 62.2  {\tiny \textcolor{blue}{(-1.7)}}& \textbf{34.6} & \textbf{36.8} & \underline{36.1} & 31.2 & \textbf{38.0} {\tiny \textcolor{red}{(+6.6)}} \\
    \bottomrule
\end{tabular}
\label{tab:asj_dsj_analysis}
\end{footnotesize}
\end{table}



==> table/Ablation3.tex <==
\noindent
\begin{table}[h]
\centering
\caption{Ratio of points remaining after LPD compared to original data. This contrasts with random drop, which exhibits a uniform remaining ratio across different distances.}
\begin{footnotesize}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    \toprule
    Distance & 0$\sim$10m & 10$\sim$20m & 20$\sim$30m & 30$\sim$40m & 40$\sim$50m & 50$\sim$60m & 60$\sim$70m & 70$\sim$80m & 80$\sim$90m \\
    \midrule
    Ratio & 80.6 & 78.6 & 78.7 & 77.4 & 76.2 & 75.5 & 76.2 & 76.4 & 72.5 \\
    \bottomrule
\end{tabular}
}
\label{tab:LPD_distance}
\end{footnotesize}
\end{table}


% \noindent
% \setlength{\tabcolsep}{0.7mm}{
% \begin{table}[t]
% \centering
% \begin{footnotesize}
% \begin{tabular}{l|ccccc|c}
%         \toprule
%         Methods & \rotatebox{90}{Clean} & \rotatebox{90}{D-fog} & \rotatebox{90}{L-fog} &  \rotatebox{90}{Rain} & \rotatebox{90}{Snow} & mIoU \\
%     \midrule
%     Baseline & \underline{63.9} & \underline{30.7} & \underline{30.1} & \textbf{29.7} & \textbf{25.3} & \textbf{31.4} \\
%     Random drop & 62.8 & 25.3 & 20.3 & 17.9 & 13.7 & 20.9 \\
%     LPD & \textbf{64.0} & \textbf{33.3} & \textbf{30.3} & \underline{28.8} & \underline{19.9} & \underline{27.3} \\
%     \bottomrule
% \end{tabular}
% \caption{Experiments on domain generalization with SemanticKITTI or SynLiDAR as source and SemanticSTF as target.}
% \label{tab:dg_stf}
% \end{footnotesize}
% \end{table}

==> table/cosmix_unimix.tex <==
\begin{table}
    \centering
    \caption{Comparison with CosMix and UniMix. DA and DG denote domain adaptation and domain generalization.}
    \begin{tabular}{cc}
        \toprule
        Methods &  mIoU \\
        \midrule
        CoSMix(DA) & 28.4 \\
        UniMix(DA) & 37.2 \\
        UniMix(DG) & 31.4 \\
        \midrule
        MinkowskiNet18+Ours & 36.3 \\
        \bottomrule
    \end{tabular}
\label{tab:compare_dgda}
\end{table}


==> table/mIoU_synlidar.tex <==
\noindent
\setlength{\tabcolsep}{0.7mm}{
\begin{table}[ht]
\centering
\caption{LiDAR segmentation results (mIoU) on the SemanticSTF~\cite{xiao_3d_2023} \textit{validation set} of models trained with SynLiDAR~\cite{xiao_transfer_2022}. $^\ast$ is the reproduced result with the same segmentation backbone. The symbol $\ddagger$ indicates that the validation for model selection was performed on sequence 0 of SynLiDAR, rather than SemanticSTF. The best score is in \textbf{bold} and the second best is \underline{underlined}.}
\scalebox{0.9}{
\begin{tabular}{l|cccc|c}
    \toprule
    Methods & \rotatebox{90}{D-fog} & \rotatebox{90}{L-fog} &  \rotatebox{90}{Rain} & \rotatebox{90}{Snow} & mIoU \\
    \midrule
    Oracle & 51.9 & 54.6 & 57.9 & 53.7 & 54.7\\ 
    \midrule
    Baseline & 15.24 & 15.97 & 16.83 & 12.76 & 15.45 \\
    LaserMix \cite{kong_lasermix_2023} & 15.32 & 17.95 & 18.55 & 13.8 & 16.85 \\
    PolarMix \cite{xiao_polarmix_nodate} & 16.47 & 18.69 & 19.63 & 15.98 & 18.09 \\
    PointDR$^\ast$ \cite{xiao_3d_2023}& \underline{19.09} & 20.28 & \underline{25.29} & \underline{18.98} & 19.78 \\
    PointDR$^\ast$$\ddagger$ & \textbf{21.41} & \underline{20.94} & \textbf{25.48} & \textbf{19.31} & \underline{20.47} \\
    \midrule
    Baseline+SJ+LPD & 19.08 & 20.65 & 21.97 & 17.27 & 20.08 \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+3.8}} & {\scriptsize \textcolor{red}{+4.7}} & {\scriptsize \textcolor{red}{+5.1}} & {\scriptsize \textcolor{red}{+4.5}} & {\scriptsize \textcolor{red}{+4.6}} \\
    Baseline+SJ+LPD$\ddagger$ & 18.99 & \textbf{21.22} & 23.14 & 17.28 & \textbf{20.51} \\
    {\scriptsize \textcolor{red}{Increments to baseline}} & {\scriptsize \textcolor{red}{+3.7}} & {\scriptsize \textcolor{red}{+5.3}} & {\scriptsize \textcolor{red}{+6.3}} & {\scriptsize \textcolor{red}{+4.5}} & {\scriptsize \textcolor{red}{+5.1}} \\
    \bottomrule
\end{tabular}
}
\label{tab:main_synlidar}
\end{table}
